How Powerful are K-hop Message Passing Graph Neural Networks

The most popular design paradigm for Graph Neural Networks (GNNs) is 1-hop message passing -- aggregating information from 1-hop neighbors repeatedly. However, the expressive power of 1-hop message passing is bounded by the Weisfeiler-Lehman (1-WL) test. Recently, researchers extended 1-hop message passing to K-hop message passing by aggregating information from K-hop neighbors of nodes simultaneously. However, there is no work on analyzing the expressive power of K-hop message passing. In this work, we theoretically characterize the expressive power of K-hop message passing. Specifically, we first formally differentiate two different kernels of K-hop message passing which are often misused in previous works. We then characterize the expressive power of K-hop message passing by showing that it is more powerful than 1-WL and can distinguish almost all regular graphs. Despite the higher expressive power, we show that K-hop message passing still cannot distinguish some simple regular graphs and its expressive power is bounded by 3-WL. To further enhance its expressive power, we introduce a KP-GNN framework, which improves K-hop message passing by leveraging the peripheral subgraph information in each hop. We show that KP-GNN can distinguish many distance regular graphs which could not be distinguished by previous distance encoding or 3-WL methods. Experimental results verify the expressive power and effectiveness of KP-GNN. KP-GNN achieves competitive results across all benchmark datasets.

==> app_kp_backup.tex <==

%\section{Proof of Theorem~\ref{thm:KP-GNN_power}}\label{app:KP-GNN_power}
%From Proposition~\ref{pro:khop_power}, we know that 1 layer $K$-hop message %passing GNN can distinguish node $v_1$ and $v_2$ whenever %$A^{k,t}_{v_1,G^{(1)}}\neq A^{k,t}_{v_2,G^{(2)}}$. The %Proposition~\ref{pro:khop_power} still holds for KP-GNN since it is $K$-hop %message passing as well. Differ from the normal $K$-hop message passing %GNNs, in each hop, a KP-GNN additionally encodes peripheral subgraph at that %hop into model. Then, it is easy to see that KP-GNN can distinguish $v_1$ %and $v_2$ if either $A^{k,t}_{v_1,G^{(1)}}\neq A^{k,t}_{v_2,G^{(2)}}$ or %$G^{k,t}_{v_1,G^{(1)}}$ and $G^{k,t}_{v_2,G^{(2)}}$ are non-isomorphic given %the message function of model. We further divide it into two situations. %(1)First, if $A^{k,t}_{v_1,G^{(1)}}\neq A^{k,t}_{v_2,G^{(2)}}$, then we have %$|Q^{k,t}_{v_1,G^{(1)}}|\neq |Q^{k,t}_{v_1,G^{(1)}}|$ at some $k \leq K$. It %means that $G^{k,t}_{v_1,G^{(1)}}$ and $G^{k,t}_{v_2,G^{(2)}}$ have %different number of nodes and thus is non-isomorphic even with 1-WL test %powerful message function. (2) if $A^{k,t}_{v_1,G^{(1)}}= %A^{k,t}_{v_2,G^{(2)}}$, we cannot distinguish two nodes by normal $K$-hop %message passing GNNs. Instead, if for some $k \leq K$, %$G^{k,t}_{v_1,G^{(1)}}$ and $G^{k,t}_{v_2,G^{(2)}}$ are non-isomorphic and %can be distinguished by $w$-WL test, then KP-GNN with a message function %that is at least powerful as $w$-WL test can also output different %representation for two peripheral subgraph, thus distinguish node $v_1$ and %node $v_2$. 

\section{Proof of Theorem~\ref{thm:kp_regular}}\label{app:kp_regular}
In this section, we prove the Theorem~\ref{thm:kp_regular}. The proof is based on NGNN~\citep{zhang2021nested} and Distance Encoding~\citep{li2020distance}. Suppose there are two $n$-node $r$-regular graphs $G^{(1)}=(V^{(1)},E^{(1)})$ and $G^{(2)}=(V^{(2)},E^{(2)})$. We pick two nodes $v_1$ and $v_2$ from each graph respectively. Assume here we use the shortest path distance kernel and the KP-GNN can only encode the information of peripheral edges, which means that the model can only distinguish two nodes if they have a different number of peripheral edges at some hops (assume no edge feature). Before we start the proof, we first introduce \textit{cross edge configuration}:
\begin{definition}
\textit{The cross edge configuration between $Q^{k,spd}_{v,G}$ and $Q^{k+1,spd}_{v,G}$ is a list $C^{k,spd}_{v,G}=(c^{1,k}_{v,G},c^{2,k}_{v,G},...)$ where $c^{i,k}_{v,G}$ denotes the number of nodes in $Q^{k+1,spd}_{v,G}$ of which each has exactly $i$ edges from $Q^{k,spd}_{v,G}$. }
\end{definition}
Note that if $C^{k,spd}_{v_1,G^{(1)}}=C^{k,spd}_{v_2,G^{(2)}}$, we have $|Q^{k+1,spd}_{v_1,G^{(1)}}|=|Q^{k+1,spd}_{v_2,G^{(2)}}|$. However, the statement is not always true if reversed. Namely, even if $|Q^{k+1,spd}_{v_1,G^{(1)}}|=|Q^{k+1,spd}_{v_2,G^{(2)}}|$, we cannot argue that $C^{k,t}_{v_1,G^{(1)}}=C^{k,t}_{v_2,G^{(2)}}$. Next, we introduce Lemma~\ref{lem:config} from Distance encoding~\citep{li2020distance}:
\begin{lemma}
\label{lem:config}
\textit{For two graphs $G^{(1)}=(V^{(1)},E^{(1)})$ and $G^{(2)}=(V^{(2)},E^{(2)})$ that are uniformly independently sampled from all $n$-node $r$-regular graphs, where $3\leq r<\sqrt{2logn}$, we pick two nodes $v_1$ and $v_2$ from two graphs respectively. Then there is at least one $i\in [\frac{1}{2}\frac{\log n}{\log(r-1-\epsilon)}, (\frac{1}{2} + \epsilon)\frac{\log n}{\log(r-1-\epsilon)}]$ with probability $1-o(n^{-1})$ such that  $C^{i,spd}_{v_1,G^{(1)}}\neq C^{i,spd}_{v_2,G^{(2)}}$. Moreover, with at least the same probability, for all $i\in [\frac{1}{2}\frac{\log n}{\log(r-1-\epsilon)}, (\frac{2}{3} - \epsilon)\frac{\log n}{\log(r-1)}]$, the number of edges between $Q_{v_j,G^{(j)}}^{i,spd}$ and  $Q_{v_j,G^{(j)}}^{i+1,spd}$  are at least $(r-1 -\epsilon) |Q_{v_j,G^{(j)}}^{i,spd}|$ for $j\in \{1,2\}$. }
\end{lemma}

The proof can be found by following steps 1-3 in the proof of Theorem 3.3 in~\cite{li2020distance}.

Now we set the $K=\lceil(\frac{1}{2} + \epsilon)\frac{\log n}{\log(r-1-\epsilon)}\rceil$ and using KP-GNN with only 1 layer. From the Lemma \ref{lem:config}, we know that with probability $1-o(n^{-1})$, there exist at least one $k< K$ with $C^{k,spd}_{v_1,G^{(1)}}\neq C^{k,spd}_{v_2,G^{(2)}}$. We select the smallest $k$ and start our proof.

\begin{enumerate}
    \item If $A^{k,spd}_{v_1,G^{(1)}}\neq A^{k,spd}_{v_2,G^{(2)}}$, then we already prove it by proposition~\ref{pro:khop_power}. Therefore, the condition we need to prove is that when $A^{k,spd}_{v_1,G^{(1)}}= A^{k,spd}_{v_2,G^{(2)}}$, which means $|Q^{k,spd}_{v_1,G^{(1)}}|=|Q^{k,spd}_{v_2,G^{(2)}}|$ for each $k=1,2,...,K$.
    \item  Next, we know that the summation of all elements in $ C^{k,spd}_{v_j,G^{(j)}}$ is equal to $|Q^{k+1,spd}_{v_j,G^{(j)}}|$ for $j\in \{1,2\}$. As we know that $|Q^{k+1,spd}_{v_1,G^{(1)}}|$=$|Q^{k+1,spd}_{v_2,G^{(2)}}|$ based on above point, $C^{k,spd}_{v_1,G^{(1)}}\neq C^{k,spd}_{v_2,G^{(2)}}$ means that the number of edge that link from nodes in $Q^{k,spd}_{v_1,G^{(1)}}$ to nodes in $Q^{k+1,spd}_{v_1,G^{(1)}}$is not equal to that of $v_2$.
    \item Meanwhile, since we are studying the regular graph, each node has the same degree. It means that the number of edge links to a given node is the same for both graph $G^{(1)}$ and $G^{(2)}$ (the node degree $r$). 
    \item The edges of node in $Q^{k,spd}_{v_1,G^{(1)}}$ must connect to nodes in either $Q^{k-1,spd}_{v_1,G^{(1)}}$, $Q^{k,spd}_{v_1,G^{(1)}}$, or $Q^{k+1,spd}_{v_1,G^{(1)}}$. This statement also holds for $G^{(2)}$. Since we have $C^{k-1,spd}_{v_1,G^{(1)}}= C^{k-1,spd}_{v_2,G^{(2)}}$ given the assumption that $k$ is the smallest value to induce different cross edge configuration, we know that the number of edge link from $Q^{k,spd}_{v_1,G^{(1)}}$ to $Q^{k-1,spd}_{v_1,G^{(1)}}$ must equal to the number of edge link from $Q^{k,spd}_{v_2,G^{(2)}}$ to $Q^{k-1,spd}_{v_2,G^{(2)}}$.
    \item Combine point 3 and 4, we conclude that the number of edge link from $Q^{k,spd}_{v_1,G^{(1)}}$ to $Q^{k,spd}_{v_1,G^{(1)}}$ is not equal to that of $v_2$, namely $|E(Q^{k,spd}_{v_1,G^{(1)}})|\neq|E(Q^{k,spd}_{v_2,G^{(2)}})|$. 
\end{enumerate}
The above statement proved that in two $r$-regular graphs, $|E(Q^{k,spd}_{v_1,G^{(1)}})|\neq|E(Q^{k,spd}_{v_2,G^{(2)}})|$ if $C^{k,spd}_{v_1,G^{(1)}}\neq C^{k,spd}_{v_2,G^{(2)}}$. Meanwhile, it is easy to see that as long as $|E(Q^{k,t}_{v_1,G^{(1)}})|\neq|E(Q^{k,t}_{v_2,G^{(2)}})|$ for some $k$, a KP-GNN with $K>k$ and only 1 layer can produce different representation for node $v_1$ and $v_2$. Combine both statements, we conclude that a KP-GNN with only peripheral edge information can produce different representation for node $v_1$ and node $v_2$ in graph $G^{(1)}$ and $G^{(2)}$.

